Planck 2015 results. V. LFI calibration

We present a description of the pipeline used to calibrate the Planck Low Frequency Instrument (LFI) timelines into thermodynamic temperatures for the Planck 2015 data release, covering four years of uninterrupted operations. As in the 2013 data release, our calibrator is provided by the spin-synchronous modulation of the cosmic microwave background dipole, but we now use the orbital component, rather than adopting the Wilkinson Microwave Anisotropy Probe (WMAP) solar dipole. This allows our 2015 LFI analysis to provide an independent Solar dipole estimate, which is in excellent agreement with that of HFI and within $1\sigma$ (0.3% in amplitude) of the WMAP value. This 0.3% shift in the peak-to-peak dipole temperature from WMAP and a global overhaul of the iterative calibration code increases the overall level of the LFI maps by 0.45% (30 GHz), 0.64% (44 GHz), and 0.82% (70 GHz) in temperature with respect to the 2013 Planck data release, thus reducing the discrepancy with the power spectrum measured by WMAP. We estimate that the LFI calibration uncertainty is now at the level of 0.20% for the 70 GHz map, 0.26% for the 44 GHz map, and 0.35% for the 30 GHz map. We provide a detailed description of the impact of all the changes implemented in the calibration since the previous data release.

==> Calibration_with_constraint.tex <==
Let $y_{i}$ be the $i$th sample of an uncalibrated data stream, and $k(i)$ the pointing period (PID) to which the sample belongs.
The toi can be modelled as
%
\begin{equation}
  y_{i} = g_{k(i)}(s_{i} +d_{i}) +b_{k(i)} +n_{i}
\end{equation}
%
where $g_{k}$ is the gain factor for $k$th pointing period, $n_{i}$ is white noise, and $b_{k}$ is an offset 
which captures the correlated noise component (or possibly an offset put there in previous data analysis steps). 
Further, $s_{i}$ is the sky signal, and $d_{i}$ is the dipole signal which includes both the cosmological component
and the component caused by satellite motion.

The sky signal can further be decomposed as
%
\begin{equation}
  s_{i} = I(\omega_{i}) +Q(\omega_{i})\cos(2\psi_{i}) +U(\omega_{i})\sin(2\psi_{i})
\end{equation}
%
where we have denoted by $\omega_i$ the pixel into which the sample falls, and by $\psi_{i}$ the orientation of polarisation sensitivity.
If polarisation is ignored, the last two term drop out.
In both cases the signal can be presented in matrix form as
%
\begin{equation}
  s_{i} = \sum_{p}P_{ip} m_{p}
\end{equation}
%
where $m$ is a map with 1 or 3 columns, depending on whether polarisation is included or not, 
and $P$ is a pointing matrix which picks the time-ordered signal from the map. 
The $i$th row of $P$ consists of all zeroes, except for the 1 or 3 elements which correspond to pixel $\omega_{i}$.

The aim is to determine the unknown quantities $m,g,b$. In particular we are interested in the gain factors $g$.
The dipole signal $d$ is assumed to be known.
Thus we want to minimize
%
\begin{equation}
  \chi^{2} = \sum_{i}\frac{1}{\sigma_{i}^{2}} ( y_{i} -y_{i}^{\mathrm{model}})^{2}  \label{chi2}
\end{equation}
%
where
%
\begin{equation}
  y_{i}^{\mathrm{model}} = g_{k(i)}(\sum_{p}P_{ip} m_{p} +d_{i}) +b_{k(i)}.  \label{ymodel}
\end{equation}
%
and $\sigma_{i}^{2}$ is the white noise variance.

We minimize (\ref{chi2}) with respect to the unknowns $m,g,b$.
Because of the quadratic form of the model ($m$ and $g$ in the same term)
we need to linearize the model, and iterate.
This can be done in multiple ways. I choose to write
%
\begin{equation}
  y_{i}^{\mathrm{model}} = g^{0}_{k(i)}\sum_{p}P_{ip} (m_{p}-m_{p}^{0})
     +g_{k(i)}(d_{i}+\sum_{p}P_{ip}m_{p}^{0}) +b_{k(i)} \label{ymodlin}
\end{equation}
%
where $g^{0}$ and $m^{0}$ are the gains and the map from the previous iteration step.
We run an iterative loop, where at every step we minimize $\chi2$ with the linearized
model (\ref{ymodlin}),
update $m^{0}$ and $g^{0}$, and repeat until convergence.

To find the minimum of $\chi^{2}$ we first rewrite the model in matrix notation.
We combine the last terms into one as
%
\begin{equation}
  g_{k(i)}(d_{i} +\sum_{p}P_{ip}m_{p}^{0})  +b_{k(i)} = \sum_{j} F_{ij} a_{j}
\end{equation}
%
Vector $a_{j}$ contains the unknowns $b$ and $g$,
and matrix $F$ spreads them into toi. 
Dipole signal $d$, and a signal picked from map $m^{0}$, are contained in $F$.

For a value of $j$ that corresponds to element $g_{k}$, we have
%
\begin{equation}
  F_{ij} = d_{i} +\sum_{p}P_{ip}m_{p}^{0}   \label{Fdef}
\end{equation}
%
if $i$ belongs to PID $k$. Other elements of the column vanish.
Similarly, when $j$ corresponds to $b_{k}$, $F_{ij}=1$ for samples that belong to that PID, zero elsewhere.

The toi model (\ref{ymodel}) can now be written in compact matrix form as
%
\begin{equation}
  \ve y^{\mathrm{model}} = \tilde P\tilde\ve m+ F\ve a.
  \end{equation}
%
where
%
\begin{equation}
  \tilde\ve m=\ve m-\ve m^{0}
\end{equation}
%
is a correction to the previous map estimate.
Gains $g^{0}$ have been transferred inside matrix $\tilde P$,
%
\begin{equation}
  \tilde P_{ip} = g^{0}_{k(i)}P_{ip}  \label{Ptilde}
\end{equation}
%
In this notation (\ref{chi2}) becomes
%
\begin{equation}
  \chi^{2} = ( \ve y -\tilde P\tilde\ve m -F\ve a)^{T} C_{n}^{-1} 
             ( \ve y -\tilde P\tilde\ve m -F\ve a)  \label{chi2mat}
\end{equation}
%
where $C_{n}$ is the white noise covariance.
Eq. (\ref{chi2mat}) is identical to the usual destriping problem, only the interpretation of the terms is different. 
In place of the pointing matrix $P$ we have $\tilde P$, which contains the gains from previous iteration step,
and $\ve a$ contains the unknown gains beside the usual baseline offsets.

We minimize (\ref{chi2mat}) with respect to $\tilde\ve m$, insert the result back,
and minimize again with respect to $\ve a$.
The solution is identical to the destriping equation
%
\begin{equation}
  \hat \ve a =   ( F^{T}C_{n}^{-1}ZF)^{-1} F^{T}C_{n}^{-1}Z\ve y  \label{destr}
\end{equation}
%
where
 %
\begin{equation}
  Z = I- \tilde P(\tilde P^{T}C_{n}^{-1} \tilde P)^{-1} \tilde P^{T} C_{n}^{-1} .\label{Zmatrix}
\end{equation}
%
We use hat to indicate that $\hat\ve a$ is an estimate of the true $\ve a$.
Eq. (\ref{destr}) can be solved by conjugate gradient iteration.
If we are interested in the gains only, this is enough. If we need also the map estimate,
it can be constructed as
 %
\begin{equation}
  \hat \ve m = (\tilde P^{T}C_{n}^{-1} \tilde P)^{-1} \tilde P^{T}C_{n}^{-1}(\ve y-F\hat\ve a)
\end{equation}
%
There are options in how the map is constructed. We may have one temperature map for each radiometer,
or two radiometers picking signal from the same signal map,
or I,Q,U maps and four radiometers looking at the same sky.


%\section{Cosmological dipole}

The dipole signal can be divided into cosmological and kinematic (satellite) component
%
\begin{equation}
  d_{i} = d_{i}^{\mathrm{sat}} +\sum_{p} P_{ip}m_{p}^{\mathrm{dip}}
\end{equation}
%
The cosmological component can be thought of as being picked from a map $\ve m^{\mathrm{dip}}$.
This has some interesting consequences.

Firstly, one readily sees that if $\ve m,\ve a$ minimize $\chi^{2}$ for a given $\ve m^{\mathrm{dip}}$,
then $\ve a, \ve m-\ve \Delta \ve m$ minimize the same quantity when $\ve m^{\mathrm{dip}}$
is replaced by $\ve m^{\mathrm{dip}}+\ve \Delta\ve m$,
since combination $\sum_{ip}P_{ip} m_{p} +d_{i}$ remains unchanged.
Thus {\it the final gains are independent of how $\ve m^{\mathrm{dip}}$ is selected}.

Secondly, consider what happens if we scale the gains by a common factor $A$.
If the kinematic dipole component was not present, we could write
%
\begin{eqnarray}
  y^{\mathrm{model}}_{i} &=& g_{k(i)}\sum_{p} (m_{p}+m_{p}^{\mathrm{dip}})  +b_{k(i)} \\
                         &=& Ag_{k(i)}\sum_{p} \left( 
                                               (m_{p} +(1-A)m_{p}^{\mathrm{dip}})/A +m_{p}^{\mathrm{dip}} 
                                                 \right) +b_{k(i)}  \nonumber
\end{eqnarray}
%
The change in $g$ could be compensated by an additional dipole component in the map.
The algorithm were then unable to determine the overall scaling of the gain, since it does not affect the goodness of the fit.
In other words, it would be impossible to determine, without additional information, if a dipole seen in the data belongs 
to the cosmological dipole, or to the sky map.
The kinematic dipole, which cannot be presented as a map, breaks the degeneracy,
but because the kinematic component is weak in comparison with the cosmological one,
we expect that {\it the overall gain level is weakly constrained}.


%\section{Dipole constraint}

Because of the degeneracy between the overall gain level and the dipole of the map,
it makes sense to constrain the map dipole.

We want to minimize $\chi^{2}$ under the additional constraint $\ve m_{c}^{T}\ve m=0$.
Here $\ve m_{c}$ is a preknown dipole map.
This is a valid assumption only if the dipole of foreground component is small.
Since most of the foreground emission comes from the galactic region,
we use a mask to exclude the galactic region from the constraint,
i.e. we set $\ve m_{c}$ to zero in the masked pixels.

We add to $\chi^{2}$ an additional prior term 
%
\begin{equation}
  \chi^{2} = ( \ve y -\tilde P\tilde\ve m -F\ve a)^{T}C_{n}^{-1} ( \ve y -\tilde P\tilde\ve m -F\ve a)
    +\ve m^{T}C_{m}^{-1}\ve m \label{chi2c}
\end{equation}
%
where we define
%
\begin{equation}
  C_{m}^{-1} = \ve m_{c}C_{d}^{-1}\ve m_{c}^{T}
\end{equation}
%
where $C_{d}$ is a constant. At the end we aim at taking the limit $C_{d}\rightarrow0$.
The prior will the force $\ve m_c^T\ve m\rightarrow0$.

Minimisation of (\ref{chi2c}) yields the solution
%
\begin{equation}
  \hat \ve a =   ( F^{T}C_{n}^{-1}ZF)^{-1} F^{T}C_{n}^{-1}Z\ve y  \label{solu1}
\end{equation}
%
with
%
\begin{equation}
  Z = I- \tilde P(M +C_{m}^{-1})^{-1} \tilde P^{T} C_{n}^{-1} \label{solu2}
\end{equation}
%
where
%
\begin{equation}
  M = \tilde P^{T}C_{n}^{-1} \tilde P.  \label{solu3}
\end{equation}
%
This differs from the original solution (\ref{destr}), (\ref{Zmatrix}) by the term $C_{m}^{-1}$ in $Z$.

Matrix $M$ is block diagonal, and can be inverted easily.
Term $C_{m}^{-1}$ breaks the block diagonal structure. We must therefore work the solution into a more practical form.
With help of Sherman-Morrison formula we find
%
\begin{eqnarray}
  (M +C_{m}^{-1})^{-1} &=& 
       (M  + \ve m_{c}C_{d}^{-1}\ve m_{c}^{T})^{-1} \\
  &=& M^{-1} -M^{-1} \ve m_{c}C_{d}^{-1} ( 1+\ve m_{c}^{T} M^{-1} \ve m_{c} C_d^{-1} )^{-1} 
               \ve m_{c}^{T}M^{-1}  \nonumber
\end{eqnarray}
%
At this point we can let $C_{d}\rightarrow0$, and the matrix simplifies into
%
\begin{equation}
  (M +C_{m}^{-1})^{-1} =
   M^{-1} -M^{-1} \ve m_{c} (\ve m_{c}^{T} M^{-1} \ve m_{c})^{-1}  \label{solu4}
               \ve m_{c}^{T}M^{-1}
\end{equation}
%
The quantity inside the brackets is a scalar, and is trivial to invert. 
One readily sees that $\ve m_{c}^{T}(M +C_{m}^{-1})^{-1}=0$,
i.e. the operation produces a map that is indeed dipole-free.

The only problem is that the constraint in the initial form has no effect on the gains.
The reason is that the monopole of the map cannot be determined from the data.
There is a perfect degeneracy between the mean of the baseline offsets $b$ and the monopole.
Therefore, the easiest way of satisfying the constraint $\ve m_{c}^{T}\ve m=0$ is to adjust the {\it monopole} of the map.
This can be done with no cost in $\chi^2$, and the algorithm always picks this solution.

To get rid of the problem it is necessary set an additional constraint for the monopole, $\ve 1^{T}\ve m=0$.
Fortunately, the mathematics for this is already in place. We just need to interpret $\ve m_{c}$ as a two-column object,
where one column is the dipole map, and another is a monopole map (constant).
The constraint $\ve m_{c}^{T}\ve m=0$ then includes both constraints.
Instead of a scalar, $\ve m_{c}^{T} M^{-1} \ve m_{c}$ becomes a $2\times2$ matrix, but it is still simple to invert.


%\section{Summary of the algorithm}

The calibration algorithm is summarized as follows.
We start from some reasonable (constant) guess for $g$.
We solve $\hat\ve a$ from Eqs. (\ref{solu1})-(\ref{solu3}), (\ref{solu4}).
We include into the procedure only the samples that fall outside the galactic region.
Object $\ve m_{c}$ is a two-column map consisting of monopole and dipole maps outside a galactic mask.
We read the gains from $\hat\ve a$, update $\tilde P$ according to (\ref{Ptilde}) and $F$ according to (\ref{Fdef}),
and repeat until the gains have converged.
This typically takes around 10 iteration steps.

The diagonal elements of $(F^{T}C_{n}^{-1}F)^{-1}$ give an estimate of the uncertainty of the gain solution.
Matrix $F^{T}C_{n}^{-1}F$ is $2\times2$ block diagonal and is simple to invert.


==> spectrum_level_rad.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4980.00,4980.00)%
    \gplgaddtomacro\gplbacktext{%
      \put(298,2862){\rotatebox{-270}{\makebox(0,0){\strut{}$-2.0$}}}%
      \put(298,3340){\rotatebox{-270}{\makebox(0,0){\strut{}$-1.0$}}}%
      \put(298,3819){\rotatebox{-270}{\makebox(0,0){\strut{}$0.0$}}}%
      \put(298,4297){\rotatebox{-270}{\makebox(0,0){\strut{}$1.0$}}}%
      \put(298,4775){\rotatebox{-270}{\makebox(0,0){\strut{}$2.0$}}}%
      \put(491,2676){\makebox(0,0){\strut{}18M}}%
      \put(886,2676){\makebox(0,0){\strut{}18S}}%
      \put(1281,2676){\makebox(0,0){\strut{}19M}}%
      \put(1676,2676){\makebox(0,0){\strut{}19S}}%
      \put(2071,2676){\makebox(0,0){\strut{}20M}}%
      \put(2466,2676){\makebox(0,0){\strut{}20S}}%
      \put(2861,2676){\makebox(0,0){\strut{}21M}}%
      \put(3256,2676){\makebox(0,0){\strut{}21S}}%
      \put(3651,2676){\makebox(0,0){\strut{}22M}}%
      \put(4046,2676){\makebox(0,0){\strut{}22S}}%
      \put(4441,2676){\makebox(0,0){\strut{}23M}}%
      \put(4836,2676){\makebox(0,0){\strut{}23S}}%
      \csname LTb\endcsname%
      \put(79,3818){\rotatebox{-270}{\makebox(0,0){\strut{}Discrepancy [\%]}}}%
      \put(4852,4589){\makebox(0,0)[r]{\strut{}$\ell \leq 50$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.00,0.00,0.00}%
      \put(298,595){\rotatebox{-270}{\makebox(0,0){\strut{}$-2.0$}}}%
      \put(298,1018){\rotatebox{-270}{\makebox(0,0){\strut{}$-1.0$}}}%
      \put(298,1441){\rotatebox{-270}{\makebox(0,0){\strut{}$0.0$}}}%
      \put(298,1863){\rotatebox{-270}{\makebox(0,0){\strut{}$1.0$}}}%
      \put(298,2286){\rotatebox{-270}{\makebox(0,0){\strut{}$2.0$}}}%
      \put(491,409){\makebox(0,0){\strut{}18M}}%
      \put(886,409){\makebox(0,0){\strut{}18S}}%
      \put(1281,409){\makebox(0,0){\strut{}19M}}%
      \put(1676,409){\makebox(0,0){\strut{}19S}}%
      \put(2071,409){\makebox(0,0){\strut{}20M}}%
      \put(2466,409){\makebox(0,0){\strut{}20S}}%
      \put(2861,409){\makebox(0,0){\strut{}21M}}%
      \put(3256,409){\makebox(0,0){\strut{}21S}}%
      \put(3651,409){\makebox(0,0){\strut{}22M}}%
      \put(4046,409){\makebox(0,0){\strut{}22S}}%
      \put(4441,409){\makebox(0,0){\strut{}23M}}%
      \put(4836,409){\makebox(0,0){\strut{}23S}}%
      \csname LTb\endcsname%
      \put(79,1440){\rotatebox{-270}{\makebox(0,0){\strut{}Discrepancy [\%]}}}%
      \csname LTb\endcsname%
      \put(2663,130){\makebox(0,0){\strut{}Radiometer}}%
      \put(4852,2100){\makebox(0,0)[r]{\strut{}$150 \leq \ell \leq 250$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{images/spectrum_level_rad.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> spectrum_level_yr.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(10200.00,5480.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.00,0.00,0.00}%
      \put(690,2944){\rotatebox{-270}{\makebox(0,0){\strut{}$-1.0$}}}%
      \put(690,4110){\rotatebox{-270}{\makebox(0,0){\strut{}$0.0$}}}%
      \put(690,5275){\rotatebox{-270}{\makebox(0,0){\strut{}$1.0$}}}%
      \csname LTb\endcsname%
      \put(471,4109){\rotatebox{-270}{\makebox(0,0){\strut{}Discrepancy [\%]}}}%
      \put(10046,5089){\makebox(0,0)[r]{\strut{}$\ell \leq 50$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.00,0.00,0.00}%
      \put(690,595){\rotatebox{-270}{\makebox(0,0){\strut{}$-1.0$}}}%
      \put(690,1566){\rotatebox{-270}{\makebox(0,0){\strut{}$0.0$}}}%
      \put(690,2536){\rotatebox{-270}{\makebox(0,0){\strut{}$1.0$}}}%
      \put(1848,409){\makebox(0,0){\strut{}1}}%
      \put(5457,409){\makebox(0,0){\strut{}2}}%
      \put(9065,409){\makebox(0,0){\strut{}3}}%
      \csname LTb\endcsname%
      \put(471,1565){\rotatebox{-270}{\makebox(0,0){\strut{}Discrepancy [\%]}}}%
      \csname LTb\endcsname%
      \put(5456,130){\makebox(0,0){\strut{}Year}}%
      \put(10046,2350){\makebox(0,0)[r]{\strut{}$150 \leq \ell \leq 250$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{images/spectrum_level_yr.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> summary_gain_plot.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(10200.00,5480.00)%
    \gplgaddtomacro\gplbacktext{%
      \put(514,3985){\rotatebox{-270}{\makebox(0,0){\strut{} 35}}}%
      \put(514,4687){\rotatebox{-270}{\makebox(0,0){\strut{} 45}}}%
      \put(514,5389){\rotatebox{-270}{\makebox(0,0){\strut{} 55}}}%
      \put(1121,3728){\makebox(0,0){\strut{}}}%
      \put(1721,3728){\makebox(0,0){\strut{}}}%
      \put(2322,3728){\makebox(0,0){\strut{}}}%
      \put(2923,3728){\makebox(0,0){\strut{}}}%
      \put(3524,3728){\makebox(0,0){\strut{}}}%
      \put(4125,3728){\makebox(0,0){\strut{}}}%
      \put(4726,3728){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(142,4696){\rotatebox{-270}{\makebox(0,0){\strut{}$K = G^{-1}$ [K\,V$^{-1}$]}}}%
      \put(5054,4100){\makebox(0,0)[r]{\strut{}A}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(656,2708){\rotatebox{-270}{\makebox(0,0){\strut{} 2}}}%
      \put(656,3168){\rotatebox{-270}{\makebox(0,0){\strut{} 4}}}%
      \put(656,3628){\rotatebox{-270}{\makebox(0,0){\strut{} 6}}}%
      \put(1121,2162){\makebox(0,0){\strut{}}}%
      \put(1721,2162){\makebox(0,0){\strut{}}}%
      \put(2322,2162){\makebox(0,0){\strut{}}}%
      \put(2923,2162){\makebox(0,0){\strut{}}}%
      \put(3524,2162){\makebox(0,0){\strut{}}}%
      \put(4125,2162){\makebox(0,0){\strut{}}}%
      \put(4726,2162){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(142,3130){\rotatebox{-270}{\makebox(0,0){\strut{}$\Delta T_\mathrm{dip}$ [mK]}}}%
      \put(5054,2534){\makebox(0,0)[r]{\strut{}B}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(514,782){\rotatebox{-270}{\makebox(0,0){\strut{} 40}}}%
      \put(514,1304){\rotatebox{-270}{\makebox(0,0){\strut{} 42}}}%
      \put(514,1826){\rotatebox{-270}{\makebox(0,0){\strut{} 44}}}%
      \put(514,2348){\rotatebox{-270}{\makebox(0,0){\strut{} 46}}}%
      \put(1121,596){\makebox(0,0){\strut{}200}}%
      \put(1721,596){\makebox(0,0){\strut{}400}}%
      \put(2322,596){\makebox(0,0){\strut{}600}}%
      \put(2923,596){\makebox(0,0){\strut{}800}}%
      \put(3524,596){\makebox(0,0){\strut{}1000}}%
      \put(4125,596){\makebox(0,0){\strut{}1200}}%
      \put(4726,596){\makebox(0,0){\strut{}1400}}%
      \csname LTb\endcsname%
      \put(142,1565){\rotatebox{-270}{\makebox(0,0){\strut{}$K$ [K\,V$^{-1}$]}}}%
      \csname LTb\endcsname%
      \put(2974,317){\makebox(0,0){\strut{}Days after launch}}%
      \put(5054,968){\makebox(0,0)[r]{\strut{}C}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5501,3914){\rotatebox{-270}{\makebox(0,0){\strut{} 8}}}%
      \put(5501,4436){\rotatebox{-270}{\makebox(0,0){\strut{} 12}}}%
      \put(5501,4957){\rotatebox{-270}{\makebox(0,0){\strut{} 16}}}%
      \put(5501,5479){\rotatebox{-270}{\makebox(0,0){\strut{} 20}}}%
      \put(6107,3728){\makebox(0,0){\strut{}}}%
      \put(6708,3728){\makebox(0,0){\strut{}}}%
      \put(7309,3728){\makebox(0,0){\strut{}}}%
      \put(7910,3728){\makebox(0,0){\strut{}}}%
      \put(8511,3728){\makebox(0,0){\strut{}}}%
      \put(9112,3728){\makebox(0,0){\strut{}}}%
      \put(9712,3728){\makebox(0,0){\strut{}}}%
      \put(10040,4100){\makebox(0,0)[r]{\strut{}A}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5643,2708){\rotatebox{-270}{\makebox(0,0){\strut{} 2}}}%
      \put(5643,3168){\rotatebox{-270}{\makebox(0,0){\strut{} 4}}}%
      \put(5643,3628){\rotatebox{-270}{\makebox(0,0){\strut{} 6}}}%
      \put(6107,2162){\makebox(0,0){\strut{}}}%
      \put(6708,2162){\makebox(0,0){\strut{}}}%
      \put(7309,2162){\makebox(0,0){\strut{}}}%
      \put(7910,2162){\makebox(0,0){\strut{}}}%
      \put(8511,2162){\makebox(0,0){\strut{}}}%
      \put(9112,2162){\makebox(0,0){\strut{}}}%
      \put(9712,2162){\makebox(0,0){\strut{}}}%
      \put(10040,2534){\makebox(0,0)[r]{\strut{}B}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5501,963){\rotatebox{-270}{\makebox(0,0){\strut{} 12.6}}}%
      \put(5501,1583){\rotatebox{-270}{\makebox(0,0){\strut{} 12.8}}}%
      \put(5501,2202){\rotatebox{-270}{\makebox(0,0){\strut{} 13}}}%
      \put(6107,596){\makebox(0,0){\strut{}200}}%
      \put(6708,596){\makebox(0,0){\strut{}400}}%
      \put(7309,596){\makebox(0,0){\strut{}600}}%
      \put(7910,596){\makebox(0,0){\strut{}800}}%
      \put(8511,596){\makebox(0,0){\strut{}1000}}%
      \put(9112,596){\makebox(0,0){\strut{}1200}}%
      \put(9712,596){\makebox(0,0){\strut{}1400}}%
      \csname LTb\endcsname%
      \put(7961,317){\makebox(0,0){\strut{}Days after launch}}%
      \put(10040,968){\makebox(0,0)[r]{\strut{}C}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{images/summary_gain_plot.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup

